Conditioning 3D Diffusion Models with 2D Images: Towards Standardized OCT Volumes through En Face-Informed Super-Resolution

High anisotropy in volumetric medical images can lead to the inconsistent quantification of anatomical and pathological structures. Particularly in optical coherence tomography (OCT), slice spacing can substantially vary across and within datasets, studies, and clinical practices. We propose to standardize OCT volumes to less anisotropic volumes by conditioning 3D diffusion models with en face scanning laser ophthalmoscopy (SLO) imaging data, a 2D modality already commonly available in clinical practice. We trained and evaluated on data from the multicenter and multimodal MACUSTAR study. While upsampling the number of slices by a factor of 8, our method outperforms tricubic interpolation and diffusion models without en face conditioning in terms of perceptual similarity metrics. Qualitative results demonstrate improved coherence and structural similarity. Our approach allows for better informed generative decisions, potentially reducing hallucinations. We hope this work will provide the next step towards standardized high-quality volumetric imaging, enabling more consistent quantifications.

==> results.tex <==
\begin{table}[!t]
\centering
\caption{Classical image similarity metrics (MSE, SSIM, and PSNR) and perceptual metrics (all LPIPS variants) calculated on the test set between the original high-resolution OCT volumes and low-resolution images that were 8$\times$ upsampled in the slice-direction using tricubic interpolation and our proposed DDIM methods. Results are presented as the mean $\pm$ standard deviation over all OCT volumes. Bolded values indicate the best values in terms of the mean performance.}
\label{tab:diffusion:quantitative}
\begin{tabular}{@{}lrrrrr@{}}



\toprule
 & Tricubic & DDIM & DDIM\textsubscript{ef} (no CFG) & DDIM\textsubscript{ef} \\ \midrule
MSE $\downarrow$ & \textbf{0.006\footnotesize{ $\pm$ 0.002}}& \textbf{0.006\footnotesize{ $\pm$ 0.003}}& \textbf{0.006\footnotesize{ $\pm$ 0.003}}& \textbf{0.006\footnotesize{ $\pm$ 0.003}} \\ 
SSIM $\uparrow$ & \textbf{0.451\footnotesize{ $\pm$ 0.116}}& 0.444\footnotesize{ $\pm$ 0.107}& 0.447\footnotesize{ $\pm$ 0.107}& 0.447\footnotesize{ $\pm$ 0.107} \\ 
PSNR (dB) $\uparrow$ & 22.472\footnotesize{ $\pm$ 1.418}& 22.401\footnotesize{ $\pm$ 1.644}& \textbf{22.495\footnotesize{ $\pm$ 1.673}}& 22.450\footnotesize{ $\pm$ 1.683} \\ \midrule
LPIPS\textsubscript{axi} $\downarrow$ & \textbf{0.120\footnotesize{ $\pm$ 0.027}}& 0.138\footnotesize{ $\pm$ 0.030}& 0.138\footnotesize{ $\pm$ 0.030}& 0.141\footnotesize{ $\pm$ 0.031} \\ 
LPIPS\textsubscript{cor} $\downarrow$ & 0.548\footnotesize{ $\pm$ 0.103}& \textbf{0.158\footnotesize{ $\pm$ 0.047}}& \textbf{0.158\footnotesize{ $\pm$ 0.048}}& 0.162\footnotesize{ $\pm$ 0.050} \\ 
LPIPS\textsubscript{sag} $\downarrow$ & 0.540\footnotesize{ $\pm$ 0.088}& \textbf{0.144\footnotesize{ $\pm$ 0.049}}& \textbf{0.144\footnotesize{ $\pm$ 0.049}}& 0.147\footnotesize{ $\pm$ 0.050} \\ 
LPIPS\textsubscript{2.5D} $\downarrow$ & 0.403\footnotesize{ $\pm$ 0.072}& \textbf{0.147\footnotesize{ $\pm$ 0.041}}& \textbf{0.147\footnotesize{ $\pm$ 0.042}}& 0.150\footnotesize{ $\pm$ 0.043} \\ 
LPIPS\textsubscript{efproj} $\downarrow$ & 0.231\footnotesize{ $\pm$ 0.055}& 0.063\footnotesize{ $\pm$ 0.039}& \textbf{0.060\footnotesize{ $\pm$ 0.039}}& 0.064\footnotesize{ $\pm$ 0.039} \\ 
\bottomrule


\end{tabular}
\end{table}

\begin{figure*}[!t]
\centerline{\includegraphics[width=.9\linewidth]{img/enface_withzoominboxes_a2.pdf}}
\caption{Examples of \enface{} projections of the OCT volumes generated using tricubic interpolation, the unconditional diffusion model \DDIM, and our proposed \enface{} conditioned diffusion model \DDIMef. These three projections are shown in the last three columns and were all generated from the 8 $\times$ downsampled (in the B-scan direction) volume as input, which is shown in the third column. The first and second rows show the corresponding high-resolution (high-res) reference and scanning laser ophthalmoscopy (SLO) image, respectively. A separate example from a different test set patient is shown in each row. The top images in each row show the full image. Zoomed-in versions of the image crops (red boxes) are shown at the bottom of each row.}
\label{fig:diffusion:enface_a}
\end{figure*}


\begin{figure*}[!ht]
\centering
\begin{subfigure}{.8\textwidth}
    \includegraphics[width=\textwidth]{img/bscan_nocond_vs_cfg_29.pdf}
    \caption{}
    \label{fig:diffusion:nocond_vs_cfg_a}
\end{subfigure}

\begin{subfigure}{.8\textwidth}
    \includegraphics[width=\textwidth]{img/bscan_nocond_vs_cfg_24.pdf}
    \caption{}
    \label{fig:diffusion:nocond_vs_cfg_b}
\end{subfigure}
\caption{Examples showing the effect of using \DDIMef, compared to leaving out the \enface{} information (\DDIM), and tricubic interpolation. In the top rows, the SLO image is shown on the left, followed by the \enface{} projections of each OCT volume. The bottom rows show zoomed-in crops. The crop locations are indicated in the top row with a lime circle. The lime horizontal line corresponds to the B-scan location from the shown crops. (a) \DDIMef reconstructs a druse that is present in the high-resolution reference, while it is missing in the OCT crops from tricubic interpolation and \DDIM. The druse also seems to be subtly visible in the SLO image. (b) The large lesion in the center of the OCT crops are more similar to the reference for \DDIMef than for tricubic interpolation and \DDIM. It is also visible in the SLO images as a hyper-intense lesion.}
\label{fig:diffusion:nocond_vs_cfg}
\end{figure*}






\begin{figure*}[!ht]
\centering

\includegraphics[width=.8\textwidth]{img/cfg_guidance.pdf}
\caption{The effect of CFG and increasing the guidance scale $w$. In the top left, the high-resolution reference is shown. In the top right, the \enface{} SLO image is shown, in which the crop location is indicated with a red box. The vertical lime lines correspond to the same physical locations throughout the figure. The horizontal lime line in the top right indicates the B-scan location of the shown OCT crops. The bottom two rows show the results from our \enface{} conditioned diffusion model with CFG for various guidance scales. $w = 0$ is equivalent to the unconditional \DDIM, $w = 1$ to \DDIMefnocfg, $w = 2$ to \DDIMef, and $w > 2$ is similar to \DDIMef, but with a larger guidance scale. The two drusen between the lime vertical lines seem to grow with a larger guidance scale.
}
\label{fig:diffusion:cfg_guidance_scale_example}
\end{figure*}



The first three rows of Table \ref{tab:diffusion:quantitative} shows the classical image similarity metrics MSE, SSIM \cite{Wang04}, and PSNR, computed between the $8 \times$ upsampled low-resolution images using DDIMs and tricubic interpolation, and the high-resolution reference images. The perceptual metrics based on LPIPS are shown in the last five rows of Table \ref{tab:diffusion:quantitative}.





For the proposed method, ablated methods and the tricubic interpolation method, we present several figures to illustrate the difference in structural similarity to the high-resolution reference images, sharpness, and coherence within the generated volumes. In Fig. \ref{fig:diffusion:enface_a} and \ref{fig:diffusion:enface_b}, we aim to point out these aspects using the \enface{} projections, allowing one to observe the overall structure of the full generated volumes. Fig. \ref{fig:diffusion:nocond_vs_cfg} and Fig. \ref{fig:diffusion:nocond_vs_cfg_continued} show additional examples of these \enface{} projections while highlighting relevant regions, alongside the corresponding image crops from the underlying OCT volume. Further examples are presented in Fig. \ref{fig:diffusion:renders}, which shows 3D renders of generated and reference volumes, and in Fig. \ref{fig:diffusion:bscan_sequences}, which shows crops of consecutive B-scans with difference maps between generated and reference images. 
Fig. \ref{fig:diffusion:difference_images} shows generation examples and difference maps for several randomly picked image crops.
The effect of increasing the guidance scale $w$ from CFG is illustrated in Fig. \ref{fig:diffusion:cfg_guidance_scale_example}. Specifically, a case of an example OCT crop is shown with several drusen that are also visible in the SLO image.





Model training took approximately 9 days on an NVIDIA A100 GPU. Sampling a full volume with 240 B-scans of 768 $\times$ 496 pixels, the most common size in the test set, resulted in 58 patches. On the aforementioned GPU type, for \DDIMef, sampling a whole volume took approximately 46 minutes. For \DDIM and \DDIMefnocfg, this sampling time was about half (approximately 23 minutes), as CFG doubles the number of required forward passes of the denoising model.

